Relevant CommonSense Subgraphs for "What if..." Procedural Reasoning

We study the challenge of learning causal reasoning over procedural text to answer "What if..." questions when external commonsense knowledge is required. We propose a novel multi-hop graph reasoning model to 1) efficiently extract a commonsense subgraph with the most relevant information from a large knowledge graph; 2) predict the causal answer by reasoning over the representations obtained from the commonsense subgraph and the contextual interactions between the questions and context. We evaluate our model on WIQA benchmark and achieve state-of-the-art performance compared to the recent models.

==> acl2022_review.tex <==
Meta Review of Paper1929 by Area Chair rAjQ 
ACL ARR 2021 November Paper1929 Area Chair rAjQ
07 Jan 2022ACL ARR 2021 November Paper1929 Meta ReviewReaders: Paper1929 Senior Area Chairs, Paper1929 Area Chairs, Paper1929 Authors, Paper1929 Reviewers, Program Chairs


Metareview:
This paper presents a subgraph extraction approach on a large (external) commonsense graph to tackle the task of procedure reasoning as a multi-hop QA task. Causal answers are predicted by learning representations for the subgraphs, contexts, and questions. Their approach was evaluated on the WIQA dataset and showed state-of-the-art performance.

Summary Of Reasons To Publish:
A new approach using subgraphs on a commonsense graph.
State-of-the-art performance on the WIQA dataset.
Summary Of Suggested Revisions:

Experiments are performed on only one dataset.

Some explanations can use good examples.

More thorough ablation studies are needed.

Overall Assessment: 3 = There are major points that may be revised




To meta-review: 
The WIQA is a special type of procedural reasoning task and the dataset has unique characteristics. That is why we focused on this data only similar to the previous papers on this problem. We hope that the contribution is clear and interesting for a short paper at ACL.
We provide the case study analysis in Figure 3 and the number of hops analysis in figure 3. Moreover, we show the ablation study in Table 3 for each component. Because of the space limitations, we don't give a more detailed explanation with examples of every part of our MRRG. Like Reviewer 2 said, the contributed MRRG approach, the application targeted, and the results are significant enough. We will add more explanation examples on the extra page and explain table 3 about the thorough ablation studies in the final version.



Official Review of Paper1929 by Reviewer DkBZ 
ACL ARR 2021 November Paper1929 Reviewer DkBZ
27 Dec 2021ACL ARR 2021 November Paper1929 Official ReviewReaders: Program Chairs, Paper1929 Senior Area Chairs, Paper1929 Area Chairs, Paper1929 Reviewers, Paper1929 Authors


Paper Summary:
The authors propose a method for relational reasoning over extracted subgraphs for multi-hop QA tasks.
They extract a subgraph by running OpenIE over the context and question and linking entities from these tuples to ConceptNet. Then, they use a context pair-wise importance score based on the contextual representation of the context + question and an encoding of each tuple extracted from ConceptNet
They select the topk tuples to construct their graph and augment its connectivity if there are edges between nodes not included as tuples.
Finally, they run a RGCN model over this graph, a BiDAF model over the context + question, and concatenate the pooled representation of the graph nodes with the output of the BiDAF model + output of a RoBERTa model to make a prediction.

Summary Of Strengths:
New model for doing multi-hop QA using extracted knowledge subgraphs
Empirical results on WIQA demonstrate improved performance over prior art
Ablation study shows the importance of different components

Summary Of Weaknesses:


Writing, not clear what exactly is done in certain steps:
Line 129: For multi token head entities, relation, and tail entities, what is the representation of each?

\cz{In line 130, we have described that we treat the triplet as a sequence and, the triplet representation is computed by the LM.}

How are E_q and E_C in line 139 computed, since these shouldn’t be single embeddings?

\cz{Sorry that this was not clear. E_q and E_C are not single embeddings. We use RoBERTa to obtain the list of token representations. $E_q$ is the list of the question tokens embeddings, while $E_C$ is the list of the paragraph tokens embeddings output of Roberta.}

Empirical study only run on one dataset
Model is quite complex
Comments, Suggestions And Typos:
N/A


Overall Assessment: 3 = Good: This paper is of interest to the *ACL audience and could be published, but might not be appropriate for a top-tier publication venue. It would likely be a strong paper in a suitable workshop.
Confidence: 4 = Quite sure. I tried to check the important points carefully. It's unlikely, though conceivable, that I missed something that should affect my ratings.
Best Paper: No
Replicability: 3 = They could reproduce the results with some difficulty. The settings of parameters are underspecified or subjectively determined, and/or the training/evaluation data are not widely available.
Datasets: 1 = No usable datasets submitted.
Software: 1 = No usable software released.
Author Identity Guess: 1 = I do not have even an educated guess about author identity.






Official Review of Paper1929 by Reviewer LBss 
ACL ARR 2021 November Paper1929 Reviewer LBss
26 Dec 2021ACL ARR 2021 November Paper1929 Official ReviewReaders: Program Chairs, Paper1929 Senior Area Chairs, Paper1929 Area Chairs, Paper1929 Reviewers, Paper1929 Authors



Paper Summary:
The paper describes a novel approach to solve the "What if.." questions when additional knowledge is needed to answer. The implementation of the approach produces state of the art 
results on the well known WIQA dataset.

Summary Of Strengths:
Well written paper with clear descriptions of each aspect of the approach Intuitive idea Presents a new way to to use the manually curated structured knowledge bases Targets the hot topic of using commonsense knowledge in the field of Natural Language Understanding.

Summary Of Weaknesses:
A running example of the problem will help in better understanding of the approach. For example, in the section 2.3: "Two entities in the triplets will have an edge if a relation r in the KG exists between them" can be better understood with the help of an example.

\cz{Because of the space limitations, we don't give a more detailed explanation with examples of every part of our MRRG. We will add more examples on the extra page in the final version.}

In section 1, it is not clear what happens if the entity out of the OpenIE system is not in the KG (ConceptNet here but I am assuming it could be any graph based KB). Mode details will be helpful

Comments, Suggestions And Typos:
More detailed explanation of every part of the approach, with examples will be helpful. It can be done by submitting the paper to a long paper instead of short because I believe the application targeted, contributed approach and the results are significant enough for a long paper.

\pk{Thank you very much for supporting the idea. We think even the one extra page of camera-ready would be good to add walk-through example if the paper accepted.}


Overall Assessment: 4 = Strong: This paper is of significant interest (for broad or narrow sub-communities), and warrants acceptance in a top-tier *ACL venue if space allows.
Confidence: 3 =  Pretty sure, but there's a chance I missed something. Although I have a good feel for this area in general, I did not carefully check the paper's details, e.g., the math or experimental design.
Best Paper: No
Replicability: 5 = They could easily reproduce the results.
Datasets: 1 = No usable datasets submitted.
Software: 5 = Enabling: The newly released software should affect other people's choice of research or development projects to undertake.
Author Identity Guess: 3 = From the contents of the submission itself, I know/can guess at least one author's name.





Official Review of Paper1929 by Reviewer n87D 
ACL ARR 2021 November Paper1929 Reviewer n87D
12 Dec 2021 (modified: 12 Dec 2021)ACL ARR 2021 November Paper1929 Official ReviewReaders: Program Chairs, Paper1929 Senior Area Chairs, Paper1929 Area Chairs, Paper1929 Reviewers, Paper1929 Authors


Paper Summary:
The paper focuses on solving the WIQA dataset, which requires model to reason over both context and commonsense graph.

The authors first encode the "question and context“, and ”the flatten ConceptNet triples" through a pre-trained language model respectively. After that, they construct a GNN on the triples to conduct multi-hop reasoning. In addition, they use a text encoder to obtain representation from the concatention of question and context.

Finally, they sumup the representation from subgraph and text encoder for a final prediction.

Summary Of Strengths:
(1) The paper propose a simple and effective system and obtain the state-of-art results on the WIQA dataset.

Summary Of Weaknesses:
(1) There is no interaction between the commonsense graph reasoning and Question-Context text encoder. Hence, the proposed model seems to be an ensemble of two indenpendent models.


\cz{In fact, our MRRG model establishes a strong interaction between the graph reasoning and text encoder via the KG attention module. As shown in Figure 2 and Section 2, we compute the context to KG triplet attention score CTS in line 143, which models the interaction. This is the reason why our MRRG model obtains the most relevant information from the graph and archives the SOTA.} 


(2) Lack a basic baseline. We can flatten the triple and then concate question, context with all triples into an input sequence for the reasoning in the pre-trained models. Without the experiement, I am not sure whether the GNN can performs better than the model with flat triples.


\cz{Indeed, this is a good baseline which the previous related work already provided. One of our strong baselines, REM-Net, uses the same idea. They use a generative model to select the triples, flatten the triples, and turned into sentences to obtain the evidence embeddings with a pre-trained encoder. Our model improves 3.46\% over REM-Net. }


Comments, Suggestions And Typos:
(1) It's more convincing to evaluate your method on a more popular dataset, such as CommonsenseQA. I find recent works[1] on CommonsenseQA adopt the entity description texts as context and also adopt the ConceptNet graph. Maybe you can use CommonsenseQA to evaluate the effectiness of your reasoning model, which combines the information from text encoder and subgraph encoder.
\pk{This is indeed interesting, however, it would be a totally different task setting. WIQA focuses on understanding a procedure/procedural reasoning which makes it distinct from commonsenseQA even if the contextual text is added there.}

[1] Fusing Context Into Knowledge Graph for Commonsense Question Answering, Xu, et al. ACL21 findings.

(2) Typo: Table 2 the font of "REM-Net (RoBERTa-large)".

Overall Assessment: 3 = Good: This paper is of interest to the *ACL audience and could be published, but might not be appropriate for a top-tier publication venue. It would likely be a strong paper in a suitable workshop.
Confidence: 4 = Quite sure. I tried to check the important points carefully. It's unlikely, though conceivable, that I missed something that should affect my ratings.
Best Paper: No
Replicability: 4 = They could mostly reproduce the results, but there may be some variation because of sample variance or minor variations in their interpretation of the protocol or method.
Datasets: 1 = No usable datasets submitted.
Software: 3 = Potentially useful: Someone might find the new software useful for their work.
Author Identity Guess: 1 = I do not have even an educated guess about author identity.




Official Review of Paper1929 by Reviewer VAmH 
ACL ARR 2021 November Paper1929 Reviewer VAmH
26 Dec 2021 (modified: 26 Dec 2021)ACL ARR 2021 November Paper1929 Official ReviewReaders: Program Chairs, Paper1929 Senior Area Chairs, Paper1929 Area Chairs, Paper1929 Reviewers, Paper1929 Authors


Paper Summary:
This paper targets at the procedure reasoning problem and focuses on the causal reansoning over the text which requires external commonsense knowlege to answer. The authors claim that there are three two challenges: (1) Effectively extracting the most relevant external information and reducing the noise from KB (2) The methods using external knowledge lacks some reasoning procedures. In order to solve the two challenges, the authors propose two methods: (1) Effectively extract a commonsense sub-graph with the most relevant information from a large knowledge graph (2) Predict the causal answers by reasoning over the representations obtained from the commonsense subgraph and the contextual interactions between the questions and context. Experimental results show that the proposed method achieved SOTA performance on WIQA dataset. Overall, this paper is easy to read and follow.

Summary Of Strengths:
1.This paper is well-written and easy to follow.

2.The experimental results achieve SOTA on WIQA datasets.

Summary Of Weaknesses:
1.The novelty of this paper is somewhat limited. The challenges and the methods to solve the problems are similar to those studies on CommonsenseQA, like (Lv et al. 2020).

\pk{The novelty of our subgraph selection is that we train the end-to-end model for it, the other related work including the referenced one that use KG, usually form a subgraph with intital entity matching and following the edges in KG in a pre-processing step. This is the main contribution of our work to choose the KG subgraph with supervision from the data.}

2.The experiments are perfomed only on one dataset. More datasets should be adopted to verify the generality of the proposed methods.

\cz{see metareview.}

Comments, Suggestions And Typos:
1.How do you select relevant external knowledge from KG? Just select the target concept from ConceptNet or other advanced methods? The attention mechanism may not be able to solve the noise problem in triples extracted from KG. What is the difference of extraction process between the this work and (Lv et al. 2020).? have you added further clarification of this point to the paper?

% \cz{subgraph adds all the entities that appear in any possible two-hop. and weakness 1}

Overall Assessment: 2.5 
Confidence: 4 = Quite sure. I tried to check the important points carefully. It's unlikely, though conceivable, that I missed something that should affect my ratings.
Best Paper: No
Replicability: 3 = They could reproduce the results with some difficulty. The settings of parameters are underspecified or subjectively determined, and/or the training/evaluation data are not widely available.
Datasets: 1 = No usable datasets submitted.
Software: 1 = No usable software released.
Author Identity Guess: 1 = I do not have even an educated guess about author identity.


We thank all reviewers for thoughtful reviewing the details of our paper and their constructive feedback. We answer to each comment individually. 

To meta-review: 
The WIQA is a special type of procedural reasoning task and the dataset has unique characteristics. That is why we focused on this data only similar to the previous papers on this problem. We hope that the contribution is clear and interesting for a short paper at ACL.
(\cz{done})

We provide the case study analysis in Figure 3 and the number of hops analysis in figure 3. Moreover, we show the ablation study in Table 3 for each component. Like Reviewer 2 said, the contributed MRRG approach, the application targeted, and the results are significant enough. 
(\cz{done})

We will add more explanation examples on the extra page and explain table 3 about the thorough ablation studies in the final version.

To reviewer 1: 
(1). In line 130, we have described that we treat the triplet as a sequence and, the triplet representation is computed by the LM. (\cz{done})

(2). Sorry that this was not clear. E_q and E_C are not single embeddings. We use RoBERTa to obtain the list of token representations. $E_q$ is the list of the question tokens embeddings, while $E_C$ is the list of the paragraph tokens embeddings output of Roberta. (\cz{done}, i rewrite the subsection.)

To reviewer 2: Because of the space limitations, we don't give a more detailed explanation with examples of every part of our MRRG. We will add more examples on the extra page in the final version. Thank you very much for supporting the idea. We think even the one extra page of camera-ready would be good to add walk-through example if the paper accepted. 

explanation with examples

To reviewer 3: (1). The novelty of our subgraph selection is that we train the end-to-end model for it, the other related work including the referenced one that use KG, usually form a subgraph with intital entity matching and following the edges in KG in a pre-processing step. This is the main contribution of our work to choose the KG subgraph with supervision from the data. (\cz{done})
(2). Please see our meta review response about the dataset.

To reviewer 4: (1). In fact, our MRRG model establishes a strong interaction between the graph reasoning and text encoder via the KG attention module. As shown in Figure 2 and Section 2, we compute the context to KG triplet attention score CTS in line 143, which models the interaction. This is the reason why our MRRG model obtains the most relevant information from the graph and archives the SOTA. (\cz{done}) Did you clarify this anywhere in the paper? 
(2). Indeed, this is a good baseline which the previous related work already provided. One of our strong baselines, REM-Net, uses the same idea. They use a generative model to select the triples, flatten the triples, and turned into sentences to obtain the evidence embeddings with a pre-trained encoder. Our model improves 3.46\% over REM-Net.  (\cz{done})
